Sustainable LLM Inference for Edge AI: Evaluating Quantized LLMs for Energy Efficiency, Output Accuracy, and Inference Latency

Deploying Large Language Models (LLMs) on edge devices presents significant challenges due to computational constraints, memory limitations, inference speed, and energy consumption. Model quantization has emerged as a key technique to enable efficient LLM inference by reducing model size and computational overhead. In this study, we conduct a comprehensive analysis of 28 quantized LLMs from the Ollama library, which applies by default Post-Training Quantization (PTQ) and weight-only quantization techniques, deployed on an edge device (Raspberry Pi 4 with 4GB RAM). We evaluate energy efficiency, inference performance, and output accuracy across multiple quantization levels and task types. Models are benchmarked on five standardized datasets (CommonsenseQA, BIG-Bench Hard, TruthfulQA, GSM8K, and HumanEval), and we employ a high-resolution, hardware-based energy measurement tool to capture real-world power consumption. Our findings reveal the trade-offs between energy efficiency, inference speed, and accuracy in different quantization settings, highlighting configurations that optimize LLM deployment for resource-constrained environments. By integrating hardware-level energy profiling with LLM benchmarking, this study provides actionable insights for sustainable AI, bridging a critical gap in existing research on energy-aware LLM deployment.

==> Figures/accuracy_table.tex <==
\begin{table}
\caption{Average Accuracy of Models on Various Datasets}
\label{tab:accuracy}
\begin{tabular}{lrrrrr}
\toprule
Dataset & bigbenchhard & commonsenseqa & gsm8k & humaneval & truthfulqa \\
Model &  &  &  &  &  \\
\midrule
gemma2\_2b\_instruct\_q3\_K\_L & 0.35 & 0.67 & 0.07 & 0.25 & 0.37 \\
gemma2\_2b\_instruct\_q3\_K\_M & 0.36 & 0.67 & 0.07 & 0.77 & 0.36 \\
gemma2\_2b\_instruct\_q3\_K\_S & 0.34 & 0.70 & 0.04 & 0.02 & 0.40 \\
llama32\_1b\_instruct\_fp16 & 0.16 & 0.35 & 0.03 & 0.62 & 0.31 \\
llama32\_1b\_instruct\_q3\_K\_L & 0.14 & 0.34 & 0.03 & 0.34 & 0.14 \\
llama32\_1b\_instruct\_q3\_K\_M & 0.10 & 0.13 & 0.03 & 0.54 & 0.03 \\
llama32\_1b\_instruct\_q3\_K\_S & 0.08 & 0.26 & 0.02 & 0.49 & 0.07 \\
llama32\_1b\_instruct\_q4\_0 & 0.20 & 0.27 & 0.05 & 0.79 & 0.39 \\
llama32\_1b\_instruct\_q4\_1 & 0.15 & 0.23 & 0.04 & 0.84 & 0.27 \\
llama32\_1b\_instruct\_q4\_K\_M & 0.23 & 0.43 & 0.06 & 0.87 & 0.34 \\
llama32\_1b\_instruct\_q4\_K\_S & 0.27 & 0.43 & 0.04 & 0.84 & 0.39 \\
llama32\_1b\_instruct\_q8\_0 & 0.17 & 0.38 & 0.04 & 0.85 & 0.34 \\
qwen25\_05b\_instruct\_fp16 & 0.27 & 0.32 & 0.04 & 0.74 & 0.23 \\
qwen25\_05b\_instruct\_q3\_K\_L & 0.28 & 0.30 & 0.03 & 0.72 & 0.31 \\
qwen25\_05b\_instruct\_q3\_K\_M & 0.26 & 0.37 & 0.07 & 0.70 & 0.24 \\
qwen25\_05b\_instruct\_q3\_K\_S & 0.20 & 0.26 & 0.01 & 0.77 & 0.31 \\
qwen25\_05b\_instruct\_q4\_0 & 0.22 & 0.28 & 0.05 & 0.72 & 0.24 \\
qwen25\_05b\_instruct\_q4\_1 & 0.28 & 0.36 & 0.07 & 0.75 & 0.29 \\
qwen25\_05b\_instruct\_q4\_K\_M & 0.25 & 0.32 & 0.06 & 0.56 & 0.26 \\
qwen25\_05b\_instruct\_q4\_K\_S & 0.25 & 0.36 & 0.08 & 0.52 & 0.26 \\
qwen25\_05b\_instruct\_q8\_0 & 0.29 & 0.32 & 0.04 & 0.54 & 0.22 \\
qwen25\_15b\_instruct\_q3\_K\_L & 0.29 & 0.45 & 0.09 & 0.03 & 0.32 \\
qwen25\_15b\_instruct\_q3\_K\_M & 0.26 & 0.40 & 0.07 & 0.02 & 0.24 \\
qwen25\_15b\_instruct\_q3\_K\_S & 0.26 & 0.57 & 0.03 & 0.17 & 0.18 \\
qwen25\_15b\_instruct\_q4\_0 & 0.33 & 0.66 & 0.09 & 0.27 & 0.24 \\
qwen25\_15b\_instruct\_q4\_1 & 0.33 & 0.67 & 0.09 & 0.08 & 0.29 \\
qwen25\_15b\_instruct\_q4\_K\_M & 0.32 & 0.62 & 0.12 & 0.20 & 0.24 \\
qwen25\_15b\_instruct\_q4\_K\_S & 0.33 & 0.57 & 0.13 & 0.18 & 0.23 \\
\bottomrule
\end{tabular}
\end{table}


==> Figures/energy_table.tex <==
\begin{table}
\caption{Mean Energy Consumption of Models on Various Datasets}
\label{tab:energy}
\begin{tabular}{lrrrrr}
\toprule
Dataset & bigbenchhard & commonsenseqa & gsm8k & humaneval & truthfulqa \\
Model &  &  &  &  &  \\
\midrule
gemma2\_2b\_instruct\_q3\_K\_L & 26.00 & 18.59 & 22.82 & 10.58 & 16.27 \\
gemma2\_2b\_instruct\_q3\_K\_M & 25.10 & 16.92 & 20.30 & 10.60 & 14.77 \\
gemma2\_2b\_instruct\_q3\_K\_S & 26.11 & 17.13 & 20.31 & 6.16 & 15.66 \\
llama32\_1b\_instruct\_fp16 & 65.50 & 32.11 & 58.45 & 13.10 & 28.69 \\
llama32\_1b\_instruct\_q3\_K\_L & 25.22 & 15.59 & 19.38 & 5.15 & 13.17 \\
llama32\_1b\_instruct\_q3\_K\_M & 25.07 & 19.30 & 15.71 & 4.39 & 21.48 \\
llama32\_1b\_instruct\_q3\_K\_S & 10.95 & 7.06 & 6.64 & 4.41 & 6.86 \\
llama32\_1b\_instruct\_q4\_0 & 28.91 & 9.09 & 11.47 & 3.71 & 8.76 \\
llama32\_1b\_instruct\_q4\_1 & 45.84 & 11.82 & 11.14 & 3.13 & 13.79 \\
llama32\_1b\_instruct\_q4\_K\_M & 36.89 & 9.18 & 12.68 & 4.18 & 9.10 \\
llama32\_1b\_instruct\_q4\_K\_S & 41.56 & 9.15 & 11.53 & 3.55 & 8.42 \\
llama32\_1b\_instruct\_q8\_0 & 36.69 & 10.57 & 18.01 & 4.84 & 9.47 \\
qwen25\_05b\_instruct\_fp16 & 13.14 & 12.44 & 8.64 & 2.10 & 7.01 \\
qwen25\_05b\_instruct\_q3\_K\_L & 10.78 & 6.84 & 4.09 & 1.05 & 3.48 \\
qwen25\_05b\_instruct\_q3\_K\_M & 5.80 & 3.52 & 3.66 & 1.02 & 3.19 \\
qwen25\_05b\_instruct\_q3\_K\_S & 13.85 & 6.61 & 3.04 & 1.81 & 3.01 \\
qwen25\_05b\_instruct\_q4\_0 & 10.85 & 5.71 & 1.98 & 1.02 & 2.80 \\
qwen25\_05b\_instruct\_q4\_1 & 9.44 & 5.82 & 3.06 & 1.15 & 3.50 \\
qwen25\_05b\_instruct\_q4\_K\_M & 8.48 & 6.69 & 4.15 & 1.22 & 4.08 \\
qwen25\_05b\_instruct\_q4\_K\_S & 7.46 & 4.54 & 4.02 & 1.13 & 4.04 \\
qwen25\_05b\_instruct\_q8\_0 & 6.60 & 6.10 & 3.50 & 1.20 & 3.49 \\
qwen25\_15b\_instruct\_q3\_K\_L & 30.15 & 15.57 & 19.37 & 4.40 & 11.25 \\
qwen25\_15b\_instruct\_q3\_K\_M & 24.11 & 15.13 & 14.88 & 3.84 & 11.55 \\
qwen25\_15b\_instruct\_q3\_K\_S & 34.32 & 15.15 & 21.34 & 0.46 & 11.42 \\
qwen25\_15b\_instruct\_q4\_0 & 21.65 & 13.35 & 12.41 & 4.02 & 9.33 \\
qwen25\_15b\_instruct\_q4\_1 & 21.88 & 13.88 & 15.37 & 3.62 & 9.29 \\
qwen25\_15b\_instruct\_q4\_K\_M & 23.42 & 14.01 & 13.57 & 4.25 & 10.60 \\
qwen25\_15b\_instruct\_q4\_K\_S & 29.05 & 13.54 & 12.92 & 3.72 & 10.19 \\
\bottomrule
\end{tabular}
\end{table}


==> accuracy_table.tex <==
\begin{table}
\caption{Average Accuracy of Models on Various Datasets}
\label{tab:accuracy}
\begin{tabular}{lrrrrrr}
\toprule
Dataset & bigbenchhard & commonsenseqa & gsm8k & humaneval & truthfulqa & Average Accuracy \\
Model &  &  &  &  &  &  \\
\midrule
gemma2\_2b\_instruct\_q3\_K\_L & 0.35 & 0.67 & 0.07 & 0.25 & 0.37 & 0.34 \\
gemma2\_2b\_instruct\_q3\_K\_M & 0.36 & 0.67 & 0.07 & 0.77 & 0.36 & 0.45 \\
gemma2\_2b\_instruct\_q3\_K\_S & 0.34 & 0.70 & 0.04 & 0.02 & 0.40 & 0.30 \\
llama32\_1b\_instruct\_fp16 & 0.16 & 0.35 & 0.03 & 0.62 & 0.31 & 0.29 \\
llama32\_1b\_instruct\_q3\_K\_L & 0.14 & 0.34 & 0.03 & 0.34 & 0.14 & 0.20 \\
llama32\_1b\_instruct\_q3\_K\_M & 0.10 & 0.13 & 0.03 & 0.54 & 0.03 & 0.17 \\
llama32\_1b\_instruct\_q3\_K\_S & 0.08 & 0.26 & 0.02 & 0.49 & 0.07 & 0.18 \\
llama32\_1b\_instruct\_q4\_0 & 0.20 & 0.27 & 0.05 & 0.79 & 0.39 & 0.34 \\
llama32\_1b\_instruct\_q4\_1 & 0.15 & 0.23 & 0.04 & 0.84 & 0.27 & 0.30 \\
llama32\_1b\_instruct\_q4\_K\_M & 0.23 & 0.43 & 0.06 & 0.87 & 0.34 & 0.39 \\
llama32\_1b\_instruct\_q4\_K\_S & 0.27 & 0.43 & 0.04 & 0.84 & 0.39 & 0.39 \\
llama32\_1b\_instruct\_q8\_0 & 0.17 & 0.38 & 0.04 & 0.85 & 0.34 & 0.35 \\
qwen25\_05b\_instruct\_fp16 & 0.27 & 0.32 & 0.04 & 0.74 & 0.23 & 0.32 \\
qwen25\_05b\_instruct\_q3\_K\_L & 0.28 & 0.30 & 0.03 & 0.72 & 0.31 & 0.33 \\
qwen25\_05b\_instruct\_q3\_K\_M & 0.26 & 0.37 & 0.07 & 0.70 & 0.24 & 0.33 \\
qwen25\_05b\_instruct\_q3\_K\_S & 0.20 & 0.26 & 0.01 & 0.77 & 0.31 & 0.31 \\
qwen25\_05b\_instruct\_q4\_0 & 0.22 & 0.28 & 0.05 & 0.72 & 0.24 & 0.30 \\
qwen25\_05b\_instruct\_q4\_1 & 0.28 & 0.36 & 0.07 & 0.75 & 0.29 & 0.35 \\
qwen25\_05b\_instruct\_q4\_K\_M & 0.25 & 0.32 & 0.06 & 0.56 & 0.26 & 0.29 \\
qwen25\_05b\_instruct\_q4\_K\_S & 0.25 & 0.36 & 0.08 & 0.52 & 0.26 & 0.29 \\
qwen25\_05b\_instruct\_q8\_0 & 0.29 & 0.32 & 0.04 & 0.54 & 0.22 & 0.28 \\
qwen25\_15b\_instruct\_q3\_K\_L & 0.29 & 0.45 & 0.09 & 0.03 & 0.32 & 0.23 \\
qwen25\_15b\_instruct\_q3\_K\_M & 0.26 & 0.40 & 0.07 & 0.02 & 0.24 & 0.20 \\
qwen25\_15b\_instruct\_q3\_K\_S & 0.26 & 0.57 & 0.03 & 0.17 & 0.18 & 0.24 \\
qwen25\_15b\_instruct\_q4\_0 & 0.33 & 0.66 & 0.09 & 0.27 & 0.24 & 0.32 \\
qwen25\_15b\_instruct\_q4\_1 & 0.33 & 0.67 & 0.09 & 0.08 & 0.29 & 0.29 \\
qwen25\_15b\_instruct\_q4\_K\_M & 0.32 & 0.62 & 0.12 & 0.20 & 0.24 & 0.30 \\
qwen25\_15b\_instruct\_q4\_K\_S & 0.33 & 0.57 & 0.13 & 0.18 & 0.23 & 0.29 \\
Average Accuracy & 0.25 & 0.42 & 0.06 & 0.51 & 0.27 & 0.30 \\
\bottomrule
\end{tabular}
\end{table}


==> approach.tex <==
\section{\sysname Framework for Monitoring Energy Consumption}
\label{sec:approach}


\begin{wrapfigure}{h}{0.550\textwidth}
    \vspace*{-1.00em}
    \centering
    \includegraphics[width=0.550\textwidth]{Figures/scaphandre-ollama-paper.drawio.pdf}
    \vspace*{-0.50em}
    \caption{Overview of the \sysname framework.}
    \label{fig:framework}
    \vspace*{-1.0em}
\end{wrapfigure}

To understand the energy consumption patterns of LLMs, we created the \sysname framework, a tool designed to monitor energy usage during the inference processes of LLMs. Figure~\ref{fig:framework} provides an architecture of this framework. 
The core of \sysname's approach involves systematically sampling prompts from a curated collection, submitting these prompts to an LLM, and recording the prompts, their responses, metadata, and the energy metrics during inference. This data is cataloged to allow for a detailed analysis of energy consumption trends during the operational phase of LLMs.




\begin{itemize}

   \item \textbf{Input Data (Prompt Dataset):} \sysname extracts prompts from a pre-existing dataset (prompt dataset in Figure~\ref{fig:framework}) and uses them to query a deployed LLM through an API client.
   
   \item \textbf{Power Usage Monitoring and Data Collection:} \sysname integrates two power monitoring tools, Scaphandre~\citep{scaphandre} and nvidia-smi~\cite{nvidia}, to track the power consumption of the deployed LLM, such as the Ollama model depicted in Figure~\ref{fig:framework}. These tools provide complementary functionalities: Scaphandre measures the CPU's power usage specific to the LLM process, while nvidia-smi assesses the total power usage of the GPU. It is crucial that no other processes operate on the GPU during LLM inference to ensure the accuracy of nvidia-smi's measurements. \sysname then calculates the energy consumption for each prompt, compiling data samples that encompass the prompt, the LLM’s response, and the associated energy metrics, thus providing a granular view of energy utilization.

   \item \textbf{Dataset Generation:} \sysname iterates through all prompts from the dataset, capturing the prompt, its response, and energy metrics. These data samples are aggregated into a comprehensive dataset, encapsulating the energy consumption of the LLM during inference.


\end{itemize}


The \sysname framework is contingent upon LLM services that can be queried for responses. While \sysname is designed to be compatible with any service offering an API endpoint for response generation, our current implementation specifically caters to services that conform to either the Ollama- or OpenAI API specifications, encapsulating the majority of prevalent LLM deployment services. These API endpoints furnish not only the LLM's natural language responses but also critical metadata, including timestamps and token lengths for both prompts and responses. The landscape of LLM deployment tools is diverse, featuring platforms such as Llama.cpp~\citep{llama.cpp}, GPT4All~\citep{anand2023gpt4all}, vLLM~\citep{kwon2023efficient}, Llamafile~\citep{llamafile}, and Ollama~\citep{ollama}. For the scope of our experiments, we chose to utilize Ollama~\citep{ollama} as our model deployment mechanism, attributing this choice to its straightforward installation process, dual compatibility with CPU and GPU architectures, and the expansive repository of open-source LLMs it supports for facile download and deployment.




Scaphandre~\cite{scaphandre} operates with process-level granularity, monitoring and recording the power usage of active processes on a computing device. We apply a regular expression to the process names to isolate the specific process associated with the LLM service. The frequency at which Scaphandre samples power metrics is configurable with granularity fine enough to reach the nanosecond scale. Although a higher sampling frequency increases the resolution and accuracy of the data, it also requires more storage for data retention and increases the energy consumption of Scaphandre itself. Therefore, we also monitor the energy consumption of Scaphandre, enabling an assessment of the energy overhead incurred by the measurement process. In contrast, nvidia-smi~\cite{nvidia} tracks the power usage of the entire GPU and lacks the capability to distinguish among multiple processes concurrently utilizing the GPU. To guarantee precise measurements, we limit the GPU to solely operating the LLM inference process. Our monitoring tools measure the power consumption $P$ of a process in microwatts ($\mu$W). We then compute the energy consumption $E$ by integrating the power consumption over the duration $t$, applying the trapezoidal rule. With $t$ expressed in seconds, we convert $E$ into kilowatt-hours (kWh) by dividing by $3.6 \times 10^{12}$, facilitating a standardized energy usage assessment.




==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


Among the various quantization techniques examined, several stand out as particularly promising for energy-efficient edge deployment. The q3\_K\_M quantization consistently delivers excellent energy efficiency across multiple model families, with qwen25\_05b\_instruct\_q3\_K\_M achieving the lowest overall energy consumption at only 1.78 J/token. This specific quantization technique appears to strike an optimal balance between aggressively reducing model size while maintaining computational efficiency.

In contrast, certain quantization techniques show inconsistent benefits. The q3\_K\_S quantization, despite using the same nominal bit precision as q3\_K\_M, yields substantially higher energy consumption in several model families. For the qwen25\_05b model, q3\_K\_S consumes 62\% more energy than q3\_K\_M, highlighting that the specific implementation details of quantization algorithms can significantly impact energy efficiency beyond the simple bit-width reduction.

From a practical deployment perspective, our findings suggest that the combination of qwen25\_05b architecture with q3\_K\_M or q4\_K\_S quantization provides the most energy-efficient option for edge devices with severe power constraints, while the gemma2\_2b models with q3\_K quantization offer a reasonable compromise when higher accuracy is required despite increased energy consumption.

==> energy_table.tex <==
\begin{table}
\caption{Mean Energy Consumption of Models on Various Datasets}
\label{tab:energy}
\begin{tabular}{lrrrrrr}
\toprule
Dataset & bigbenchhard & commonsenseqa & gsm8k & humaneval & truthfulqa & Average Energy per Token (J/tok) \\
Model &  &  &  &  &  &  \\
\midrule
gemma2\_2b\_instruct\_q3\_K\_L & 26.00 & 18.59 & 22.82 & 10.58 & 16.27 & 18.85 \\
gemma2\_2b\_instruct\_q3\_K\_M & 25.10 & 16.92 & 20.30 & 10.60 & 14.77 & 17.54 \\
gemma2\_2b\_instruct\_q3\_K\_S & 26.11 & 17.13 & 20.31 & 6.16 & 15.66 & 17.07 \\
llama32\_1b\_instruct\_fp16 & 65.50 & 32.11 & 58.45 & 13.10 & 28.69 & 39.57 \\
llama32\_1b\_instruct\_q3\_K\_L & 25.22 & 15.59 & 19.38 & 5.15 & 13.17 & 15.70 \\
llama32\_1b\_instruct\_q3\_K\_M & 25.07 & 19.30 & 15.71 & 4.39 & 21.48 & 17.19 \\
llama32\_1b\_instruct\_q3\_K\_S & 10.95 & 7.06 & 6.64 & 4.41 & 6.86 & 7.19 \\
llama32\_1b\_instruct\_q4\_0 & 28.91 & 9.09 & 11.47 & 3.71 & 8.76 & 12.39 \\
llama32\_1b\_instruct\_q4\_1 & 45.84 & 11.82 & 11.14 & 3.13 & 13.79 & 17.14 \\
llama32\_1b\_instruct\_q4\_K\_M & 36.89 & 9.18 & 12.68 & 4.18 & 9.10 & 14.41 \\
llama32\_1b\_instruct\_q4\_K\_S & 41.56 & 9.15 & 11.53 & 3.55 & 8.42 & 14.84 \\
llama32\_1b\_instruct\_q8\_0 & 36.69 & 10.57 & 18.01 & 4.84 & 9.47 & 15.92 \\
qwen25\_05b\_instruct\_fp16 & 13.14 & 12.44 & 8.64 & 2.10 & 7.01 & 8.67 \\
qwen25\_05b\_instruct\_q3\_K\_L & 10.78 & 6.84 & 4.09 & 1.05 & 3.48 & 5.25 \\
qwen25\_05b\_instruct\_q3\_K\_M & 5.80 & 3.52 & 3.66 & 1.02 & 3.19 & 3.44 \\
qwen25\_05b\_instruct\_q3\_K\_S & 13.85 & 6.61 & 3.04 & 1.81 & 3.01 & 5.66 \\
qwen25\_05b\_instruct\_q4\_0 & 10.85 & 5.71 & 1.98 & 1.02 & 2.80 & 4.48 \\
qwen25\_05b\_instruct\_q4\_1 & 9.44 & 5.82 & 3.06 & 1.15 & 3.50 & 4.59 \\
qwen25\_05b\_instruct\_q4\_K\_M & 8.48 & 6.69 & 4.15 & 1.22 & 4.08 & 4.92 \\
qwen25\_05b\_instruct\_q4\_K\_S & 7.46 & 4.54 & 4.02 & 1.13 & 4.04 & 4.24 \\
qwen25\_05b\_instruct\_q8\_0 & 6.60 & 6.10 & 3.50 & 1.20 & 3.49 & 4.18 \\
qwen25\_15b\_instruct\_q3\_K\_L & 30.15 & 15.57 & 19.37 & 4.40 & 11.25 & 16.15 \\
qwen25\_15b\_instruct\_q3\_K\_M & 24.11 & 15.13 & 14.88 & 3.84 & 11.55 & 13.90 \\
qwen25\_15b\_instruct\_q3\_K\_S & 34.32 & 15.15 & 21.34 & 0.46 & 11.42 & 16.54 \\
qwen25\_15b\_instruct\_q4\_0 & 21.65 & 13.35 & 12.41 & 4.02 & 9.33 & 12.15 \\
qwen25\_15b\_instruct\_q4\_1 & 21.88 & 13.88 & 15.37 & 3.62 & 9.29 & 12.81 \\
qwen25\_15b\_instruct\_q4\_K\_M & 23.42 & 14.01 & 13.57 & 4.25 & 10.60 & 13.17 \\
qwen25\_15b\_instruct\_q4\_K\_S & 29.05 & 13.54 & 12.92 & 3.72 & 10.19 & 13.88 \\
Average Energy per Token (J/tok) & 23.74 & 11.98 & 13.37 & 3.92 & 9.81 & 12.57 \\
\bottomrule
\end{tabular}
\end{table}


==> subjects.tex <==
\subsection{Experiment Design}
\label{sec:subjects}


\textbf{Datasets}.
Datasets...


\noindent \textbf{Experimental setup}. Experimental setup...


